HAVOK Model Predictive Control for Time-Delay Systems with Applications to District Heating

A computationally efficient Model-Predictive Control (MPC) approach is proposed for systems with unknown delay using only input/output data. We use the Koopman operator framework and the related Hankel Alternative View of Koopman (HAVOK) algorithm to identify a model in a basis of projected time-delay coordinates and demonstrate a novel MPC structure that reduces and bounds the computational complexity. The proposed HAVOK-MPC approach is validated experimentally on a laboratory-scale District Heating System (DHS), demonstrating excellent prediction and tracking performance while only requiring knowledge of a conservative upper bound on the system delay.

==> Sections/Discussion.tex <==
Discuss plz

==> Sections/HAVOK_for_Input_Delayed_Systems.tex <==
Is this ok?

==> Sections/Simulation.tex <==
To verify the practicability of the proposed control design, we first simulate a single-supplier, dual-consumer system using the equations described in \cref{subsec:DHS}. To emulate a mixing loop with a local controller rather than a directly controllable heat source, \cref{eq:TempInModel} is replaced by a first-order model with a fast heating regime and slow cooling regime corresponding to the transfer functions:

\begin{equation}\label{eq:MixingLoopDyn}
	G_{HEAT}(s) = \frac{\frac{1}{93}}{s+\frac{1}{93}}, \quad G_{COOL}(s) = \frac{\frac{1}{173}}{s+\frac{1}{173}}
\end{equation}

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=8.4cm]{Figures/DHSMPCRelaxed}    % The printed column width is 8.4 cm.
		\caption{HAVOK-MPC tracking performance in simulation environment. Note that only the distal, actively controlled consumer temperature is depicted.} 
		\label{fig:HAVOKSim}
	\end{center}
\end{figure}

Data is collected from a single simulation where the mixing loop setpoint is perturbed over its entire operating range, with both setpoint values and setpoint intervals uniformly distributed. Respectively the setpoint and the distal consumer temperature are sampled at $T_s = 1\text{s}$, then downsampled to $T_{MPC} = 60\text{s}$, while flow rate is kept constant throughout. A HAVOK model is then constructed with $n_d = 20$ and $r = 5$,  as per \cref{eq:HAVOK}, and a HAVOK-MPC setpoint controller is designed according to \cref{eq:MSMPCIntegratorCausal} and implemented using YALMIP (\cite{Lofberg:2004}). Weighting matrices $Q$ and $R$ were chosen by iteration; we remark that the entries in $Q$ corresponding to states in PCT coordinates must generally be chosen very large relative to the setpoint deviation weight as they are inherently numerically small, and we propose that it may be expedient to pre-weight these modes with the singular values.

The controller is evaluated on a $3$-setpoint trajectory over $12$ hours. Results are seen on \cref{fig:HAVOKSim}, and we note excellent performance during both heating and cooling, with no overshoot during heating and very limited undershoot during cooling despite a clearly visible transport delay of over $5$ minutes and mixing loop dynamics that cannot instantaneously track the MPC setpoint $u_{MPC}$.
